Arnold: an eFPGA-Augmented RISC-V SoC for Flexible and Low-Power IoT End-Nodes

A wide range of Internet of Things (IoT) applications require powerful, energy-efficient and flexible end-nodes to acquire data from multiple sources, process and distill the sensed data through near-sensor data analytics algorithms, and transmit it wirelessly. This work presents Arnold: a 0.5 V to 0.8 V, 46.83 uW/MHz, 600 MOPS fully programmable RISC-V Microcontroller unit (MCU) fabricated in 22 nm Globalfoundries GF22FDX (GF22FDX) technology, coupled with a stateof-the-art (SoA) microcontroller to an embedded Field Programmable Gate Array (FPGA). We demonstrate the flexibility of the System-OnChip (SoC) to tackle the challenges of many emerging IoT applications, such as (i) interfacing sensors and accelerators with non-standard interfaces, (ii) performing on-the-fly pre-processing tasks on data streamed from peripherals, and (iii) accelerating near-sensor analytics, encryption, and machine learning tasks. A unique feature of the proposed SoC is the exploitation of body-biasing to reduce leakage power of the embedded FPGA (eFPGA) fabric by up to 18x at 0.5 V, achieving SoA state bitstream-retentive sleep power for the eFPGA fabric, as low as 20.5 uW. The proposed SoC provides 3.4x better performance and 2.9x better energy efficiency than other fabricated heterogeneous re-configurable SoCs of the same class.

==> arnold.include.tex <==


\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}

%custom shortcuts
\newcommand{\io}{I/O}


%area numbers
\newcommand{\effectiveArea}{4.11mm\textsuperscript{2}}

\newcommand{\socareanoefpga}{1.11mm\textsuperscript{2}}
\newcommand{\udmaarea}{21755.14$\mu$m\textsuperscript{2}}
\newcommand{\memarea}{734232.02$\mu$m\textsuperscript{2}}
\newcommand{\riscyarea}{27030.94$\mu$m\textsuperscript{2}}
\newcommand{\efpgasubsyarea}{63945.52$\mu$m\textsuperscript{2}}

%relative percentage
\newcommand{\udmapercarea}{2\%}
\newcommand{\mempercarea}{66.2\%}
\newcommand{\riscypercarea}{2.5\%}
\newcommand{\efpgasubsyperarea}{5.8\%}

\newcommand{\fcbpercarea}{6.3\%}
\newcommand{\dcfifopercarea}{5.1\%}
\newcommand{\mathpercarea}{84.9\%}

\newcommand{\risckyPMParea}{3718.64\mu$\textsuperscript{2}}
\newcommand{\risckyPMPovh}{14\%}
\newcommand{\risckyFPUDParea}{3172.64$\mu$\textsuperscript{2}}
\newcommand{\risckyFPURFarea}{2764.60$\mu$\textsuperscript{2}}
\newcommand{\risckyFPUarea}{5937.24$\mu$\textsuperscript{2}}
\newcommand{\risckyFPUovh}{22\%}

\newcommand{\FPGACPUACCcycles}{114327}

\newcommand{\FPGAAREAspipulpino}{24\%}
\newcommand{\FPGAAREAmuntaniala}{12\%}
\newcommand{\FPGAAREAbnnacc}{42\%}
\newcommand{\maxFLL}{2.1GHz}

%Acronyms
\acrodef{ASIC}{Application specific integrated circuit}
\acrodef{FPGA}{Field Programmable Gate Array}
\acrodef{MCU}{Microcontroller unit}
\acrodef{SoC}{System-On-Chip}
\acrodef{CPU}{Central Processing Unit}
\acrodef{API}{Application Programming Interface}

\acrodefplural{ASIC}[ASICs]{Application specific integrated circuits}
\acrodefplural{FPGA}[FPGAs]{Field Programmable Gate Arrays}
\acrodefplural{MCU}[MCUs]{Microcontroller units}
\acrodefplural{SOC}[SoCs]{System-On-Chips}
\acrodefplural{API}[APIs]{Application Programming Interfaces}

\acrodef{NTC}{Near-Threshold Computing}
\acrodef{FDSOI}{Fully Depleted   Silicon-On-Insulator}
\acrodef{ADC}{Analog-to-Digital converter}
\acrodef{AFE}{analog front-end}
\acrodef{DSP}{digital signal processor}
\acrodef{AP}{Action Potential}
\acrodef{EEG}{Electroencephalography}
\acrodef{LFP}{Local Field Potential}
\acrodef{SoA}{\textit{State-of-the-art}}
\acrodef{PPA}{Power-Performance-Area}
\acrodef{DWT}{\textit{Discrete Wavelet Transform}}
\acrodef{ISA}{Instruction Set Architecture}
\acrodef{PMP}{Physical Memory Protection}
\acrodef{ROM}{read-only-memory}
\acrodef{SRAM}{static random-access-memory}
\acrodef{APB}{AMBA Advanced Peripheral Bus}
\acrodef{GF22FDX}{Globalfoundries GF22FDX}
\acrodef{MAC}{Multiply-and-Accumulate}
\acrodef{FLL}{Frequency-locked loop}
\acrodef{FCB}{Fabric Configuration Block}
\acrodef{OTS}{Off-the-Shelf}
